Modular constructive Lyndon interpolation for nondistributive logics

We establish the Lyndon interpolation property for basic lattice expansion logics (LE-logics) in arbitrary signatures using display calculi. Our approach is constructive, yielding interpolants algorithmically from derivations, and modular, in the sense that interpolation for axiomatic extensions can be obtained by verifying a local interpolation property for the analytic structural rules corresponding to the additional axioms. To this end, we identify a class of interpolation-safe structural rules preserving local Lyndon interpolation. As applications of the general framework, we show that the tense version of Holliday's fundamental modal logic enjoys the Lyndon interpolation property.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> packages.tex <==
\let\openbox\relax
\let\proof\relax
\let\endproof\relax

%AiML packages

%\usepackage{aimlmacro}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{authblk}
\usepackage{amsthm}

%%%

\usepackage{lscape}
\usepackage{pdflscape}


\usepackage{stmaryrd}
\usepackage{mathdots}

%\usepackage[greek.ancient,english]{babel}
%\usepackage[greek,english]{babel}
\usepackage[geometry]{ifsym}
\usepackage{cmll}

\usepackage{comment}
%\usepackage{proof}

%\usepackage{eucal}
\usepackage{amscd}
\usepackage{amssymb}

%\usepackage{amsthm}
%\usepackage{mathptmx}
\usepackage{mathrsfs}

\usepackage{color}
\usepackage{xspace}
\usepackage{bussproofs}
\EnableBpAbbreviations

%\usepackage[single]{accents}
%\usepackage{graphicx}
%\usepackage{amscd}

%\usepackage{unicode-math}
\usepackage{mathtools}
%\setmathfont{XITS math}


%\usepackage{amssymb,amsmath}
%%%\usepackage{mathptmx}
%\usepackage{mathrsfs}


%\usepackage{tikz}



\usepackage{enumerate}

\usepackage{centernot}


%\usepackage{mathtools}



\usepackage{hyperref}

\usepackage{cleveref}

%\usepackage{relsize}

\usepackage{caption}

\usepackage{multirow}

%\usepackage{multicol}

\usepackage{array}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{L}[1]{>{\arraybackslash}p{#1}}




%\usepackage{graphics}
\usepackage{color}
\usepackage{cancel}
%\usepackage{stmaryrd}
%%\usepackage{amssymb,amsmath}
%\usepackage{amsthm}
%[nointegrals]
%\usepackage{proof}
\usepackage{verbatim,cmll}
\usepackage{setspace}
\usepackage{lscape}
\usepackage{latexsym,relsize}
%\usepackage{amscd}
\usepackage{multicol}
%\usepackage{bussproofs}
%\EnableBpAbbreviations

\usepackage[position=top]{subfig}
%\usepackage{leqno}
\usepackage{tikz}

\usepackage{txfonts}

%\usepackage{authblk}
\usepackage{multicol}
\usetikzlibrary{arrows}
\usetikzlibrary{matrix}
\usetikzlibrary{patterns}
\usetikzlibrary{shapes}
%\usepackage[bb=boondox]{mathalfa}
%\usepackage{enumerate}
\usepackage{marginnote}
